Controllable Textual Inversion for Personalized Text-to-Image Generation

The recent large-scale generative modeling has attained unprecedented performance especially in producing high-fidelity images driven by text prompts. Text inversion (TI), alongside the text-to-image model backbones, is proposed as an effective technique in personalizing the generation when the prompts contain user-defined, unseen or long-tail concept tokens. Despite that, we find and show that the deployment of TI remains full of "dark-magics" -- to name a few, the harsh requirement of additional datasets, arduous human efforts in the loop and lack of robustness. In this work, we propose a much-enhanced version of TI, dubbed Controllable Textual Inversion (COTI), in resolving all the aforementioned problems and in turn delivering a robust, data-efficient and easy-to-use framework. The core to COTI is a theoretically-guided loss objective instantiated with a comprehensive and novel weighted scoring mechanism, encapsulated by an active-learning paradigm. The extensive results show that COTI significantly outperforms the prior TI-related approaches with a 26.05 decrease in the FID score and a 23.00% boost in the R-precision.

==> sections/append-experiment.tex <==
\section{Appendix}

\subsection{Implementation Details for Aesthetic Scorers}
% 对ReLIC和TANet, 我们微调
% 对Chad Scorer，image encoder做表征接全连接层

\subsection{Experimental Settings}

To verify the effectiveness and extensibility and of our proposed \NAME{} framework, we conduct experiments on 8 different concepts that the large-scale text-to-image (i.e. Stable Diffusion~\cite{rombach2022high}) do not involve and implement different versions of \NAME{}.
This section explains some important implementation details for the dataset, the aesthetic scorer, the concept-matching scorer we use, and how we design the learning paradigm. 

\paragraph{Datasets.}
To focus on concepts that the text-to-image models do not involve, we need to specifically collect data relevant to these concepts. In terms of data collection, we took the following steps.
First, we collect 8 concepts that hardly be generated through prompt engineering on the text-to-image model, in which we the concepts are manually grouped into 4 pairs, indicating that concepts within one group are somehow similar.% including axolotl, frilled_lizard, crampfish, garfish, emperor_penguin_chick, king_penguin_chick, indian_cobra, sidewinder
Then, we collect images related to the given concepts crawled from publicly available internet and also collect images from other open-source datasets with consistent category labels.
Be aware that this web-crawled dataset is uncurated, we manually select 10~(out of 1,000 images with in each concept) images of the highest quality to form the initial training set and assign an aesthetic score of 10 to each of them~(since aesthetic scores typically range from 1 to 10).
% Be aware that this large-scale dataset is uncurated. Keep in mind that the uncurated nature of the dataset means that collected links may lead to strongly discomforting and disturbing content for a human viewer
% Including fixed dataset like ImageNet, iNaturalist 2018~\cite{van2018inaturalist}, IP102~\cite{wu2019ip102}
% Including image host websites including baidu, Dreamstime, Flicker, isotckphoto, pinterest, shutterstock

\paragraph{Aesthetic Scorers.} To offer the basic knowledge for aesthetic evaluation, we use pre-trained generic models, including ReLIC~\cite{zhao2020representation}, TANet~\cite{he2022rethinking} and SD-Chad Scorer. Note that the scores given by generic aesthetic scoring model tends to lie in the majority score range (5~6) in our dataset, we ought to personalize this model accordingly to our training set, which we refer to as PIAA~\cite{zhu2020personalized}. Since PIAA is a typical small sample problem, we adopt similar experimental settings and evaluation criteria by referring Few-Shot Learning~\cite{fe2003bayesian} and a previous PIAA research work: PA-IAA~\cite{li2020personality}.

\paragraph{Concept-Matching Scorers.} Since the first step of general image-retrieval is the feature extraction, we use the image encoder within our text-to-image model, which it is trained over billions of text-image pairs and can be regarded as reliable feature extractors. Meanwhile, diffusion-based models are also widely used as good feature extractors in image-retrieval~\cite{donoser2013diffusion,bai2018regularized,zhao2018modelling,liu2019guided}. We adopt three version of retrieval scores, i.e. VLAD, Set Distance and Classification.

\paragraph{Active Learning Procotol.} For all experiments, we start from a initial training set $\mathbf{X}_T$ with 10 manually and carefully selected samples, while the web-crawled set $D_W$ contains 1,000 samples. Then, we perform $K$ cycles of the following actions (with $K$ at most 20): (1) Train the scoring system based on the training set $\mathbf{X}_T$ and auxiliary sets $D_{TG}$ and $D_{SI}$, in which $|\mathbf{X}_T|=|D_{TG}|=|D_{SI}|$ and we regenerate $D_{TG}$ and reselect $D_{SI}$ at the beginning of the cycle; (2) Train the embedding on $\mathbf{X}_T$ with each sub-cycle with $I=1,000$ epochs, and save an embedding per $I_{step}=50$ epochs. Beginning with learning rate $5\times 10^{-4}$, the sub-cycles are continuously conducted with the learning rate is lowered down only when the best embedding is not the latest version. Our learning rates include $5\times 10^{-4},2.5\times 10^{-4},7.5\times 10^{-5},5\times 10^{-5},2.5\times 10^{-5}$. The cycle ends when the learning rate reaches the minimum value and the embedding quality cannot be further boosted. (3) Select top-10 samples according to the embedding score and the dual scoring system from web-crawled set $D_W$ and add them to $\mathbf{X}_T$.

\begin{table*}[t]
    \centering
    \caption{\textbf{Experimental results of different strategies on 8 concepts}. We compare our dual selective active training strategy with random selection and with full dataset. It is obvious that out proposed method significantly outperforms any of them. Furthermore, we also show the priority of our method with generated images in Figure~\ref{fig:main_score_fig}.}
    \vspace{0.5em}
    \begin{tabular}{l|ccccc}
        \toprule
        \multirow{2}{*}{Concepts} & \multicolumn{5}{c}{Performance(R-precision)} \\ \cmidrule{2-6}
                                & RAND             & FULL             & RAND(scheduled)               & FULL(scheduled)            & \textbf{\NAME{}} \\ \midrule
         axolotl                & 62.35$\pm$3.56\% & 63.39$\pm$4.15\% & 69.56$\pm$2.23\% & 72.57$\pm$3.23\% & \textbf{92.36$\pm$1.29\%} \\
         frilled lizard         & 54.39$\pm$4.68\% & 58.23$\pm$5.43\% & 62.33$\pm$1.97\% & 68.39$\pm$2.55\% & \textbf{91.39$\pm$2.04\%} \\
         crampfish              & 70.37$\pm$2.33\% & 68.37$\pm$4.04\% & 72.35$\pm$2.56\% & 76.56$\pm$2.44\% & \textbf{94.23$\pm$2.85\%} \\
         garfish                & 72.55$\pm$3.08\% & 72.37$\pm$2.93\% & 75.62$\pm$1.03\% & 75.23$\pm$1.88\% & \textbf{90.26$\pm$1.55\%} \\
         emperor penguin(chick) & 58.36$\pm$0.98\% & 55.23$\pm$2.04\% & 68.94$\pm$2.33\% & 70.03$\pm$1.97\% & \textbf{88.06$\pm$0.99\%} \\
         king penguin(chick)    & 60.36$\pm$2.58\% & 61.25$\pm$1.93\% & 65.65$\pm$1.92\% & 64.14$\pm$0.76\% & \textbf{86.23$\pm$0.73\%} \\
         indian cobra           & 67.23$\pm$2.88\% & 65.24$\pm$4.05\% & 70.26$\pm$1.03\% & 72.35$\pm$0.99\% & \textbf{87.56$\pm$1.43\%} \\
         sidewinder             & 62.42$\pm$5.06\% & 63.12$\pm$4.23\% & 68.39$\pm$3.67\% & 69.12$\pm$1.23\% & \textbf{85.24$\pm$1.12\%} \\ \bottomrule
    \end{tabular}
    \label{tab:main_score}
\end{table*}

\begin{figure*}[ht]
\centering
\vspace{-1em}
\includegraphics[width=0.9\textwidth]{iccv2023AuthorKit/images/comparison.pdf}
\caption{\textbf{A comparison of generated images of different strategies on 8 concepts}. We can see that our proposed \NAME{} consistently produce better images than any other strategies, when the single-score-based strategies work better than random selection and full dataset but still face problems in capturing some visual details of the concept.}
\label{fig:main_score_fig}
\end{figure*}

\subsection{Comparison with different strategies.}\label{exp:compare}

\begin{table}[t]
    \centering
    \caption{\textbf{Experimental Results on emperor penguin~(chicks) with different variants for the dual scorer within \NAME{}.} Concept-matching scorer has 3 variants, i.e. ReLIC, TANet and SD-Chad while aesthetic scorer has 3 variants: VLAD, Set Distance(Set), and Classification(CLASS). All the variants are evluated by R-precision(\%) with dual selective active training.} 
    \vspace{0.5em}
    \resizebox{0.9\linewidth}{!}{\begin{tabular}{l | ccc}
    \toprule
    \multirow{2}{*}{\makecell[c]{Matching \\ Score}} & \multicolumn{3}{c}{Aesthetic Score} \\
     & ReLIC & TANet & SD-Chad \\ \midrule
     VLAD  & 84.45$\pm$2.43 & 85.23$\pm$0.92 & 85.66$\pm$1.23 \\
     Set   & 82.36$\pm$1.27 & 87.73$\pm$0.98 & 87.03$\pm$1.35 \\
     CLASS & 86.67$\pm$0.24 & 85.35$\pm$1.03 & \textbf{88.06$\pm$0.99} \\ \bottomrule
    \end{tabular}}
    \includegraphics[width=0.9\linewidth]{iccv2023AuthorKit/images/comparison_version.pdf}
    \label{tab:different_versions}
\end{table}

We compare our proposed method with random selection~(RAND) and full dataset without any selection~(FULL). Meanwhile, we also test RAND and FULL with the dynamic schedule to further see how selection impacts the framework.
All the embeddings are finally evaluated through R-precision~\cite{xu2018attngan}, a common evaluation metric for ranking retrieval results.
For each generated image, we use $R$ corresponding text descriptions and another $1000R$ randomly selected unmatched descriptions to form a text description pool~(which are also prompts modified from ImageNet), with other detailed consistent with CPGAN~\cite{liang2020cpgan}.% Compute the cosine similarity between the text features and the image features for each description. Sorted according to the similarity, the real description falls in the top-R is considered correct, otherwise it is wrong. If there are r results in top-R that are image-related (that is, they can describe the image correctly), then R-precision is r/R.
%  The implementation detailed are explained in the supplementary material.

\paragraph{\NAME{} consistently and significantly outperforms other strategies.} The experimental results can be seen in Table~\ref{tab:main_score} and Figure~\ref{fig:main_score_fig}, in which our proposed \NAME{} significantly outperforms other baselines on all concepts within the dataset. On concept frilled lizard, our proposed active selection strategy can achieve 23\% R-precision boost, while others also achieve more than 15\% performance boost. The main reason for such a large performance gap is that \NAME{} captures the two important factor~(i.e. aesthetics and object clarity) that impact the quality of the embeddings, while other simple strategies (even with assistance from schedules) ignore how they impact the embedding. These results experimentally prove the necessity of specifically design a dual selective paradigm for embedding training in personalized text-to-image generation. % Further results on how individual score influences the training will be presented in Sec.~\ref{exp:ablation}.
We also test several variants of \NAME{} by applying different aesthetic scorer and concept-matching scorers, with experimental results shown in Figure~\ref{tab:different_versions}. Since \NAME{} with Chad Scorer and classifier-based matching shows the best result, we use this version to compare with other methods.

In addition, we observe that random selection~(RAND) sometimes even outperforms the full dataset~(like crampfish, emperor penguin chicks and indian cobra), which is also consistent with our observation in Figure~\ref{fig:intro_example_comparison_2}. We account this for the potential low-quality samples~(i.e. low-resolution, excessive disturbing objects) within web-crawled dataset. Even with a dynamic schedule, these harmful details cannot be eliminated~(as shown in Figure~\ref{fig:main_score_fig}). These results further verify the importance of carefully selecting training samples for personalized text-to-image generation.

\begin{figure*}[t]
    \vspace{-0.5em}
    \centering
    \subfigure[The number of epochs with specified different learning rates within the schedule on RAND.]{\includegraphics[width=0.23\textwidth]{iccv2023AuthorKit/images/bar_proportion_rand.png}}
    \hspace{0.5em}
    \subfigure[The number of epochs with specified different learning rates within the schedule on \NAME{}.]{\includegraphics[width=0.23\textwidth]{iccv2023AuthorKit/images/bar_proportion_dasatti.png}}
    \hspace{0.5em}
    \subfigure[Changes on different score as cycle proceeds on RAND.]{\includegraphics[width=0.23\textwidth]{iccv2023AuthorKit/images/plot_curve_class_rand.png}}
    \hspace{0.5em}
    \subfigure[Changes on different score as cycle proceeds on \NAME{}.]{\includegraphics[width=0.23\textwidth]{iccv2023AuthorKit/images/plot_curve_class_dasatti.png}}
    \caption{\textbf{A comparison on how the schedule and scores change on RAND(scheduled) and \NAME{} as cycle proceeds on concept emperor penguin(chick).} (a),(b) show how the \#epochs for each learning rate in the schedule change as cycle proceeds, when (c),(d) show how aesthetic/concept-matching/comprehensive score change on RAND(scheduled) and \NAME{}. The scores for \NAME{} stop changing at cycle 12 since more added samples do not help boost embedding quality.}
    \label{fig:schedule_score_compare}
\end{figure*}

\paragraph{\NAME{} is more reliable on schedules.} % training epochs and learning rate
Figure~\ref{fig:schedule_score_compare}(a),(b) show a comparison on how our schedules adjusts as the number of cycles increase on RAND(scheduled) and \NAME{}. Both of them shows the tendency that training epochs with larger learning rates decrease when those with small learning rate increases, meaning that the training schedule shown in \ref{method:dual_selective_active_training} focus more on fine-tuning at later cycles. Comparing \NAME{} with RAND, we can see that the epochs with the maximal learning rate already diminish at cycle 4 on \NAME{} while RAND still needs large learning rates, indicating that \NAME{} are better at recognize the given concept and tends to be more stable.

\paragraph{\NAME{} achieves an good score earlier than other methods.} Figure~\ref{fig:schedule_score_compare}(c),(d) shows a comparison on how the aesthetic/concept-matching/comprehensive scores change as cycle proceeds on RAND and \NAME{}. We can see that \NAME{} already achieve higher value on all scores and cannot be further boosted with 120 training samples on cycle 12 when the performance for RAND still fluctuates. This phenomena illustrates that our active selection strategy make our embedding be trained on more high-quality data.

Furthermore, we also notice that aesthetic/concept-matching scores fluctuates at later cycles when the comprehensive score is enhanced continuously, which exactly corresponds to our proposed dual scoring system that balance the importance of these two factors, when ensuring the quality of embedding never declines.

\subsection{Ablation Studies}\label{append_exp:ablation}

We verify the effectiveness of all components in our proposed \NAME{} framework on concept "emperor penguin(chick)", which includes the scoring models, embedding scoring within the dual scoring system, and the dynamic schedule designed according to the dual scorer. The results are shown as follows.

\begin{table}[h]
    \centering
    \caption{\textbf{R-precision(\%) of \NAME{} compared with other single-score based strategies.} We apply a dynamic training schedule to all the strategies here for a fair comparison, with $\mathcal{N}_L$ denoting the size of the training data. The results are produced with 9 single-score strategies to see the impact of generation-based, aesthetic-based and retrieval-based scores.} 
    \vspace{0.5em}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|c|cc}
        \toprule
        \multicolumn{2}{c|}{Method} & $\mathcal{N}_T=50$ & $\mathcal{N}_T=200$ \\ \midrule
        \multicolumn{2}{c|}{Random} & 45.67$\pm$5.66 & 68.94$\pm$2.33 \\ \midrule
        \multirow{3}{*}{\makecell[c]{Single Score \\ (Generation)}} 
        & IS & 46.39$\pm$4.05 & 67.31$\pm$2.34 \\
        & FID & 52.19$\pm$2.33 & 67.45$\pm$1.89 \\
        & LPIPS & 51.39$\pm$2.58 & 70.89$\pm$2.46 \\ \midrule
        \multirow{3}{*}{\makecell[c]{Single Score \\ (Aesthetic)}} 
        & ReLIC & 60.98$\pm$1.37 & 75.67$\pm$3.06 \\
        & TANet & 56.05$\pm$2.03 & 74.23$\pm$2.93 \\
        & SD-Chad & 60.24$\pm$0.36 & 77.65$\pm$1.86 \\ \midrule
        \multirow{3}{*}{\makecell[c]{Single Score \\ (Retrieval)}}
        & VLAD & 60.03$\pm$1.75 & 76.28$\pm$2.24 \\
        & Set Distance & 59.67$\pm$1.93 & 77.28$\pm$0.36 \\
        & Classification & 61.78$\pm$2.55 & 78.45$\pm$1.09 \\ \midrule
        \multicolumn{2}{c|}{\NAME{}(without dual scorer)} & 66.03$\pm$3.45 & 85.45$\pm$1.04 \\
        \multicolumn{2}{c|}{\NAME{}} & \textbf{69.08$\pm$2.03} & \textbf{88.06$\pm$0.99} \\
    \bottomrule
    \end{tabular}}
    \label{tab:single_score_comparison}
\end{table}

\begin{figure}[t]
\centering
\vspace{-1em}
\includegraphics[width=0.9\linewidth]{iccv2023AuthorKit/images/test_plot_curve_class_r_precision.png}
\caption{\textbf{R-precision(\%) with different strategies as training pool expands.} The experiments are performed over concept "emperor penguin(chick)" and produced over RAND and \NAME{}. To further show the impact of the number of samples, we also compare their modified versions that do not use dynamic schedules.}
\label{fig:on_num_samples}
\end{figure}

\paragraph{Comparing with other score-based selection or single score}. First, we validate the effectiveness of our dual scoring system by comparing it with single-score based selection in Table~\ref{tab:single_score_comparison}, which include generation-based score, aesthetic score and concept-matching score, with all the experiments equipped with the dynamic scheduling in Sec.~\ref{method:dual_selective_active_training} for fair comparison. Generation-based scores include evaluation metric for generative models like inception score~(IS)~\cite{salimans2016improved}, and learned perceptual image patch similarity~(LPIPS)~\cite{zhang2018unreasonable}, which can also be used for selection.

In Table~\ref{tab:single_score_comparison}, we can see the aesthetic/retrieval-based strategies consistently outperform the scores induced from generation-based evaluation metrics. We account this for that those metrics focus on a generic generation scheme rather than focusing on a given concept, making them unsuitable for in this setting. We can also see that the dual scoring strategy in \NAME{} consistently outperforms the single-score-based ones (i.e. 7.30\% with 50 training samples and 9.61\% with 200 training samples) on different data scales.
From these comparisons, we claim that design scoring systems especially design for personalized text-to-image generation is important, and our dual scoring system exactly meet this requirement with an dual image selection strategy which adjusts the scoring preference according to the embeddings.

In addition, we also test how \NAME{} behaves when we do not discriminate the score for embedding evaluation and image selection~(by setting both $S_{dual}(e)$ and $S_{dual}(x)$ to Eq.~\ref{eq:embedding_generated_image}). We can also see a 3.05\% performance drop with 50 training samples and a 2.61\% drop with 200 samples. This phenomenon confirms the importance of adjusting sample scores according to embeddings.


%\paragraph{The impact the introducing embedding scores into scoring system.}

\paragraph{The effect of dynamic scheduling.} 
To look at the influence of an active training paradigm, we also compare the performance of RAND and \NAME{} with their schedule-fixed versions in Figure~\ref{fig:on_num_samples}. 
We can see that without a dynamic schedule, both RAND and \NAME{} faces performance loss or fluctuation with much more samples (i.e., 100 samples for \NAME{} and 120 samples for RAND). For RAND, more samples do not necessarily give preciser visual descriptions for a concept, which in turn leads to inferiority compared to other sampling methods. For \NAME{}, samples at later cycles tends to have lower quality~(i.e. lower resolution, disturbing elements), which can include redundant or even harmful details, which can be alleviated via dynamic schedules. To conclude, our dual selective active training paradigm is also essential for obtaining good embeddings.

\subsection{Further Extension: Concept with multiple shapes}

\begin{figure}[t]
\centering
\vspace{-1em}
\includegraphics[width=0.9\linewidth]{iccv2023AuthorKit/images/multi_form.pdf}
\caption{\textbf{A comparison on real-images with \NAME{}-generated ones in 3 different shapes of lycorma delicatula.} We can see that with a carefully designed active selective training framework, the embedding helps produce all the shapes of the concept "lycorma delicatula".}
\label{fig:on_different_shapes}
\end{figure}

Recall that Stable Diffusion 2.0 fails to generate emperor penguin chicks, which accounts for the fact that adult emperor penguin chicks and their chicks have different appearance. We raise another question: can we train an embedding with a concept that have different shapes? Inspired by this, we also test our proposed \NAME{} on concept “lycorma delicatula”, which is a kind of pest with 3 different forms in its life-cycle, and surprisingly find that with 300 training samples, the best version of embeddings successfully produces all these 3 shapes, as shown in Figure~\ref{fig:on_different_shapes}. These results further validate the effectiveness of our framework, even in the presence of appearance  ambiguity.

\section{Details}

In this section, we describe our proposed \FULLNAME{}~(\NAME{}) framework in detail. Initially, we have web-crawled dataset $D_W$ related to the concept given, and a manually selected training dataset $\mathbf{X}_T$. All the images in $\mathbf{X}_T$ are of high quality~(i.e. aesthetically good enough when the object is also clear), when $\mathbf{X}_T$ might contain distorted images or even mismatch the given concept, which is common in web-crawled data.

In traditional active learning, we train all the models we use on the training set $\mathbf{X}_T$. Then, we select a batch of data $B$ from web-crawled dataset $D_W$ according to the acquisition functions induced from models. Finally, we move this selected batch of data $B$ to $\mathbf{X}_T$, go back to the model training step to re-train or fine-tune the models and repeat this cycle until $\mathbf{X}_T$ reach its maximum capacity or the quality of models cannot be enhanced by adding new data.

\subsection{Overview}

% first paragraph: overview for scoring system
We use a dual scoring system as the acquisition module that both evaluate the quality of images and embeddings in our proposed \NAME{} framework. In traditional active learning or data selection, the acquisition module is only conducted on samples. However, based on the prior experiment shown in Figure~\ref{fig:intro_example_comparison_2}, we know that an increase on the number of samples do not necessarily contribute to performance boost like traditional active learning setting. Therefore, we propose this dual scoring system to help schedule embedding training, select the best version among them, and select samples accordingly to their quality.

% second paragraph: overview for dynamic schedule according to scoring system
Instead of using a fixed learning schedule in embedding training, we leverage the scoring system and include two informative cues, \textit{aesthetic score} and \textit{concept-matching score}, in embedding quality evaluation and selection. Moreover, to avoid introducing unnecessary details like watermarks, borders or disturbing objects, we design a dynamic training schedule that adjust itself according to the quality score for the current embedding. Then, based on the carefully trained embedding, samples that may further enhance its quality from the web-crawled dataset are also selected accordingly.

% last paragraph: summarize the whole framework
As shown in Figure~\ref{fig:dati}, our \FULLNAME{} framework can be divided into 4 steps: (1) Train the scoring system on the current training set $\mathbf{X}_T$ (Sec.~\ref{method:scoring_system}). (2) Train the textual inversion embedding on the training set $\mathbf{X}_T$ and schedule the training accordingly to the scoring system (Sec.~\ref{method:embedding_selection},\ref{method:schedule}); (3) Select the best version of embedding, and calculate the acquisition score accordingly to the scoring system and the best embedding for samples in web-crawled datset $D_W$ (Sec.~\ref{method:data_selection}); (4) Select top-K samples from $D_W$ and move them to training set $\mathbf{X}_T$.

\subsection{Scoring system}\label{method:scoring_system}

We attribute the quality of an image/embedding to two factors: \textit{aesthetics} and \textit{concept-matching}, which are also two key points quantifying how the input image affects the embedding.
As a long-standing field, "aesthetics" comprehensively considers whether the lighting, contrast, texture and other photographic factors of an image are consistent with human aesthetics.
"Concept-matching" is adopted from image retrieval, which is originally used to retrieve an object image containing a corresponding concept, and we use it to detect whether the object is clear enough to describe a concept. An ideal image consists of objects clear enough and good photographic attributes, while an ideal embedding procedures ideal images.
Our scoring system we designed takes both these two points into consideration for both images/embeddings, and the details are listed as follows.

\subsubsection{Aesthetic Scorer}\label{method:aesthetic_scorer}

The general aesthetic scorer is described as follows:
\begin{equation}
    p=S_{aes}(x,\theta),
\end{equation}
where $S_{aes}$ indicates the aesthetic scoring model, $p$ denotes the predicted score, and $x$ represents the input image, with $\theta$ denote the model parameters. Since we focus on one concept in this setting, we personalize an aesthetic scorer for this concept based a pre-trained generic aesthetic model. Following the work of PA-IAA~\cite{li2020personality}, we directly ﬁne-tune the generic aesthetic model with our training data to learn personalized preference.
% generic aesthetic model can be: ReLIC, TANet, Chad Scorer

To make model distinguish bad/good examples within this concept, we carefully design the aesthetic training set $\mathbf{X}_T^{aes}$based on $\mathbf{X}_T$. In this work, the aesthetics training comprises of three parts: (1) The original training set $\mathbf{X}_T$; (2) Generated set $D_{TG}$ without assistance from any embeddings; (3) Randomly sampled set $D_{SI}$ from similar categories.
Since we focus on the concepts that the text-to-image model can hardly recognize and visualize, $D_{TG}$ contains lots of plausible, disrupted or even irrelevant samples, which we assign zero score. This helps the aesthetic model understand that originally generated samples are "bad samples". In contrast, $D_{SI}$ somehow describes some attributes for the concept, but still does not match the concept, which we assign the average score. We employ the normal regression loss formulated as follows:
\begin{equation}
    \mathcal{L}_{aes}=\frac{1}{|\mathbf{X}_T|}\sum_{x_t\in \mathbf{X}_T}\Vert p_t, \hat{p}_t\Vert+\frac{\lambda}{|D_{TG}|}\sum_{x'_t\in D_{TG}\cup D_{SI}}\Vert p'_t - \hat{p}'_t\Vert,
\end{equation}
where $\hat{p}$ denotes the ground-truth label we assign, and $\lambda$ is set to 1 in our experiments. In this manner, the score personalized for this concept for each sample from $D_W$ can be predicted from the aesthetic scorer.

% the large-scale text-to-image already presents a good image encoder, so we can use this encoder to extract image features, this is how chad scorer is designed.

\subsubsection{Concept Matching Scorer}\label{method:concept_matching_scorer}

Since concept-matching in image retrieval are typically conducted on feature maps, we directly use the image encoder within the text-to-image model as the feature extractors and give out the matching score accordingly to the corresponding representation space. Let $R_T=\{r_1,r_2,\dots,r_{|\mathbf{X}_T|}\}$ be the feature map set extracted from $\mathbf{X}_T$, a concept-matching scorer $S_{con}$ can be formulated as:
\begin{equation}
    S_{con}(x)=\frac{1}{|\mathbf{X}_T|}\sum_{k=1}^{|\mathbf{X}_T|}\phi\left(r_x, r_k\right),
\end{equation}
where $r_x$ denotes the representation given by image-encoder on the given samples $x$, when function $\phi(r_x,r_k)$ is used to measure the similarity between sample $x$ and feature map $r_k$.

People has proposed several variants for $\phi(\cdot,\cdot)$ in this similarity evaluation, including VLAD~\cite{jegou2010aggregating}, Set distance~\cite{iscen2018mining} and Classification~\cite{boudiaf2020unifying}, which we modified to fit into our concept matching scorer:
\begin{itemize}
    \item By setting $\phi\left(r_x, r_k\right)=\psi(r_x, r_k)\exp\left(-\Vert r_x-r_k\Vert\right)$, where $\psi(r_x, r_k)=1$ if $r_k$ is the closet representation for $r_k$ and is set to 0 otherwise. VLAD regards the extracted representations for $\mathbf{X}_T$ as a codebook and maps each image to its nearest code.
    \item Set difference mines correlated samples by comparing their set distance, where $S_{con}(x)=\exp\left(-\min_{\mathbf{X}_T\in R_T}\Vert d_x - \mathbf{X}_T\Vert\right)$.
    \item Classification locates relevant samples by attaching and training another fully-connected network to the image coder and performs binary classification. By regarding $\mathbf{X}_T$ as positive samples and $D_{TG}\cup D_{SI}$ (proposed in~\ref{method:aesthetic_scorer}) as negative sample set, this can also be achieved with probabilistic outputs.
\end{itemize}
Note that samples within $\mathbf{X}_T$ are guaranteed to be clean and clear samples, this score is sufficient to quantify whether the object~(if exists) in the given image distinguish itself from other photographic components and match the given concept.

\subsubsection{Dual Scorer}\label{method:dual_scorer}

After calculating the aesthetic score and concept-matching score for each image, we combine these terms to form the final information score $S_{dual}(x)=F\left(S_{aes}(x), S_{con}(x)\right)$, where $F$ denotes a combination scheme and can be adjusted to serve different purposes~(with details explained in the following section). Meanwhile, note that the quality of embeddings can also be judged by their generated images, we also evaluate an embedding $e$ with this scoring system:
\begin{equation}
    S_{dual}(e)=\frac{1}{D_e}\sum_{x_e\in D_e}S_{dual}(x_e),
    \label{eq:embedding}
\end{equation}
where $D_e$ is the set of images generated by the text-to-image model according to embedding $e$.
At this stage, since the scoring system can both evaluate the quality of individual images and embeddings, we name this a "dual scorer".
% whether dual space theories can be added?

\subsection{Dual Selective Active Training}\label{method:dual_selective_active_training}

With the scoring system completed above, we are able to conduct our dual selective active training paradigm.
A naive way to incorporate the scoring system into the active learning paradigm is to use a fixed training schedule and move the top-ranked samples from $D_W$ to $\mathbf{X}_T$ for the next training cycle. Nevertheless, this strategy also results in unnecessary details or incorrect elements introduced into embeddings, as shown in Figure~\ref{fig:intro_example_comparison_2}. Though the scoring system does select samples with good quality, it fails to find samples that can further enhance the embedding. 
% 是否要配图强调如果不用动态的paradigm，而是单纯地根据得分选样本且schedule固定会怎么样

Since embedding evaluation and data acquisition serves different objectives, we apply different schemes when scoring embedding/samples. In particular, a good embedding should procedure images with both high aesthetics and object clarity, when good images for the next cycle should make up for the final embedding at the current cycle. 
To better select samples that further enhance the quality of embeddings, we propose a dual selective active training paradigm that couples embedding evaluation/selection and data acquisition as follows.

\subsubsection{Embedding Evaluation and Selection}\label{method:embedding_selection}
We measure the quality of an embedding through the aesthetic scores and concept-matching scores on its generated data batch, in which these two factors are equally important.
Given a embedding set $E=\{e_1,e_2,\dots,e_v\}$, we generate a evaluation set $D_{e_i}$ for each embedding $e_i$. Then, we use the dual scoring system to calculate the quality score for each generated data point:
\begin{equation}
    S_{dual}(x_e)=10\sin\left(\frac{\pi}{20}S_{aes}\left(e\right)\right)\sin\left(\frac{\pi}{20}S_{con}\left(e\right)\right). \label{eq:embedding_generated_image}
\end{equation}
% provide illustrations for using this function
This function changes rapidly when individual scores become close to 5.0, when 5.0 is exactly the average score that scorers tend to offer to most images, consistent with our need to quickly distinguish good examples from average ones. When one score draws near 10.0, the dual scorer become less sensitive to this score and will focus more on another factor. Last and perhaps more important, this score attains higher value when the two scores becomes close, which explicitly emphasize that embeddings that balancing the two factors are of better quality.
With the embedding score deduced then calculated according to Eq.~\ref{eq:embedding}, we manage to select the best version of embedding $e^*=\argmax_{e\in E}S_{dual}(e)$ among the embedding set $E$.

\subsubsection{Embedding Training Schedule}\label{method:schedule}

As the number of training samples increases, the quality of selected samples at later cycles might be lower, and a fixed schedule may introduce some unnecessary details within these images~(such as watermarks, borders, disturbing objects, etc.). But these subsequent samples with relatively lower quality do contain some good photographic that can help the embedding evolve. Actually, the potential problems can be alleviated by carefully-designed schedules.

We first train the embedding for $I$ epochs, and save an embedding version $e_i$ per $I_{step}$ epochs, together with its corresponding generated images, constituting a sub-cycle. When this sub-cycle is completed, we filter out the embedding with the highest quality based on the score in Sec.~\ref{method:embedding_selection}. If the selected embedding has the most training epochs across all versions, we keep the learning rate and conduct the next sub-cycle, otherwise we will reduce the learning rate. 
Note that if the embedding quality of this cycle is not as good as that of the previous cycle (because of the quality degradation caused by introducing some unnecessary details), the initial learning rate will be reduced, which help avoid introducing disturbing elements led by some samples with insufficient quality.
The sub-cycles will be continuously conducted until the minimum learning rate is reached or the embedding quality no longer increases.
The cycle in in Figure \ref{fig:intro_example_comparison_2}(b) offers an intuitive illustration for how \NAME{} make the schedule.

\subsubsection{Data Acquisition}\label{method:data_selection}

After getting the final embedding $e$ by carefully scheduling embedding training and selecting the best version among them, we select the most suitable samples for the next-cycle training.
Notice that whether newly selected images enhance the embedding depends on both the quality and the embedding, we ought to adjust our preferences according to the embedding. In more detail, when the embedding has high aesthetics but does not guarantee object clarity, samples with high concept-matching scores better enhance the embedding; when the embedding fails to exhibit some photographic attributes consistent with human, samples with high aesthetics are preferred. To implement this preference, our acquisition score for data in web-crawled set is:
\begin{equation}
    \begin{aligned}
        S_{dual}(x) &= (1-\sin(\frac{\pi}{20}S_{aes}(e)))S_{aes}(x) \\
        &+ (1-\sin(\frac{\pi}{20}S_{con}(e)))S_{con}(x).
    \end{aligned}
\end{equation}

After selecting top-K data accordingly to this score based on embedding quality, we assign a lowered aesthetic score to them:
\begin{equation}
    \hat{p}_x = 10.0 - \frac{N_{current}}{N_{total}}(10.0 - p_x),
\end{equation}
where $p_x$ denotes the score given by a generic aesthetic scorer, $N_{total}$ represents the number of total active learning cycles, when $N_{current}$ indicates the current cycle. Note that the newly-selected images typically have lower quality than those from earlier cycles, we assign progressively lowered score to them as learning cycle proceeds.

Finishing the active selection step for both embedding and next-cycle images, we repeat the loop above to fine-tune the scorers and the embedding on the updated training set $\mathbf{X}_T$.

\begin{algorithm}[t]
	\caption{An active learning cycle for \NAME{}.}
	\label{alg:cycle_dati}
	\KwIn{Text-to-image model $g(\cdot)$, web data pool $W$, training data pool $\mathbf{X}_T$, budget $B$, pretrained aesthetic scorer $S_{aes}(\cdot,\theta)$, concept-matching scorer $S_{con}(\cdot)$, text embedding $v$, learning rate group $R$.}
	\KwOut{Updated training pool $\mathbf{X}_T$, updated embedding $v$.}  
	\BlankLine
 
        % for data selection
        Fine-tune the aesthetic scorer $S_{aes}(\cdot,\theta)$ on $\mathbf{X}_T$;
        
        % Calculate the score for embedding
        Calculate the aesthetic score $\gamma_{aes}(v)$ (Eq.~\eqref{eq:vec_aes}) and concept-matching score $\gamma_{con}(v)$ (Eq.~\eqref{eq:vec_con}) for $v$;

        \ForEach{$x_w\in W$}{
            Calculate the integrated score $S_{int}(x)$(Eq.~\eqref{eq:score_integration});
        }
        $\mathcal{B}\leftarrow$\{Top-B samples within $W$ according to $S_{int}$\};
        
        % for training
        $s\leftarrow \gamma(v)$~(Eq.~\eqref{eq:embedding_final_score});
        
        $r\leftarrow$ the largest value within $R$;
        
        \While{$r\neq \min(R)$}{
            $v'\leftarrow v-r\nabla_v\sum_{x\in \mathbf{X}_T\cup\mathcal{B}}L_{LDM}(x,v)$;

            Generate a small-scale $X_{TI}$ with $g(\cdot)$ conditioned on $v'$; 
            
            Calculate score $\gamma(v)$ for $v$ via Eq.~\eqref{eq:embedding_final_score} and $X_{TI}$;

            \uIf{$\gamma(v) > s$}{
                $v\leftarrow v'$;
                
                $s\leftarrow \gamma(v)$;
            }
            \Else{
                $r\leftarrow$ a smaller value than $r$ within $R$;
            }
	}
 
        $\mathbf{X}_T\leftarrow \mathbf{X}_T\cup\mathcal{B}$
\end{algorithm}




\iffalse

In this section, we describe our proposed \FULLNAME{}~(\NAME{}) framework in detail. Initially, we have web-crawled dataset $D_W$ related to the concept given, and a manually selected training dataset $\mathbf{X}_T$. All the images in $\mathbf{X}_T$ are of high quality~(i.e. aesthetically good enough when the object is also clear), when $\mathbf{X}_T$ might contain distorted images or even mismatch the given concept, which is common in web-crawled data.

In traditional active learning, we train all the models we use on the training set $\mathbf{X}_T$. Then, we select a batch of data $B$ from web-crawled dataset $D_W$ according to the acquisition functions induced from models. Finally, we move this selected batch of data $B$ to $\mathbf{X}_T$, go back to the model training step to re-train or fine-tune the models and repeat this cycle until $\mathbf{X}_T$ reach its maximum capacity or the quality of models cannot be enhanced by adding new data.

\subsection{Overview}

% first paragraph: overview for scoring system
We use a dual scoring system as the acquisition module that both evaluate the quality of images and embeddings in our proposed \NAME{} framework. In traditional active learning or data selection, the acquisition module is only conducted on samples. However, based on the prior experiment shown in Figure~\ref{fig:intro_example_comparison_2}, we know that an increase on the number of samples do not necessarily contribute to performance boost like traditional active learning setting. Therefore, we propose this dual scoring system to help schedule embedding training, select the best version among them, and select samples accordingly to their quality.

% second paragraph: overview for dynamic schedule according to scoring system
Instead of using a fixed learning schedule in embedding training, we leverage the scoring system and include two informative cues, \textit{aesthetic score} and \textit{concept-matching score}, in embedding quality evaluation and selection. Moreover, to avoid introducing unnecessary details like watermarks, borders or disturbing objects, we design a dynamic training schedule that adjust itself according to the quality score for the current embedding. Then, based on the carefully trained embedding, samples that may further enhance its quality from the web-crawled dataset are also selected accordingly.

% last paragraph: summarize the whole framework
As shown in Figure~\ref{fig:dati}, our \FULLNAME{} framework can be divided into 4 steps: (1) Train the scoring system on the current training set $\mathbf{X}_T$ (Sec.~\ref{method:scoring_system}). (2) Train the textual inversion embedding on the training set $\mathbf{X}_T$ and schedule the training accordingly to the scoring system (Sec.~\ref{method:embedding_selection},\ref{method:schedule}); (3) Select the best version of embedding, and calculate the acquisition score accordingly to the scoring system and the best embedding for samples in web-crawled datset $D_W$ (Sec.~\ref{method:data_selection}); (4) Select top-K samples from $D_W$ and move them to training set $\mathbf{X}_T$.

\subsection{Scoring system}\label{method:scoring_system}

We attribute the quality of an image/embedding to two factors: \textit{aesthetics} and \textit{concept-matching}, which are also two key points quantifying how the input image affects the embedding.
As a long-standing field, "aesthetics" comprehensively considers whether the lighting, contrast, texture and other photographic factors of an image are consistent with human aesthetics.
"Concept-matching" is adopted from image retrieval, which is originally used to retrieve an object image containing a corresponding concept, and we use it to detect whether the object is clear enough to describe a concept. An ideal image consists of objects clear enough and good photographic attributes, while an ideal embedding procedures ideal images.
Our scoring system we designed takes both these two points into consideration for both images/embeddings, and the details are listed as follows.

\subsubsection{Aesthetic Scorer}\label{method:aesthetic_scorer}

The general aesthetic scorer is described as follows:
\begin{equation}
    p=S_{aes}(x,\theta),
\end{equation}
where $S_{aes}$ indicates the aesthetic scoring model, $p$ denotes the predicted score, and $x$ represents the input image, with $\theta$ denote the model parameters. Since we focus on one concept in this setting, we personalize an aesthetic scorer for this concept based a pre-trained generic aesthetic model. Following the work of PA-IAA~\cite{li2020personality}, we directly ﬁne-tune the generic aesthetic model with our training data to learn personalized preference.
% generic aesthetic model can be: ReLIC, TANet, Chad Scorer

To make model distinguish bad/good examples within this concept, we carefully design the aesthetic training set $\mathbf{X}_T^{aes}$based on $\mathbf{X}_T$. In this work, the aesthetics training comprises of three parts: (1) The original training set $\mathbf{X}_T$; (2) Generated set $D_{TG}$ without assistance from any embeddings; (3) Randomly sampled set $D_{SI}$ from similar categories.
Since we focus on the concepts that the text-to-image model can hardly recognize and visualize, $D_{TG}$ contains lots of plausible, disrupted or even irrelevant samples, which we assign zero score. This helps the aesthetic model understand that originally generated samples are "bad samples". In contrast, $D_{SI}$ somehow describes some attributes for the concept, but still does not match the concept, which we assign the average score. We employ the normal regression loss formulated as follows:
\begin{equation}
    \mathcal{L}_{aes}=\frac{1}{|\mathbf{X}_T|}\sum_{x_t\in \mathbf{X}_T}\Vert p_t, \hat{p}_t\Vert+\frac{\lambda}{|D_{TG}|}\sum_{x'_t\in D_{TG}\cup D_{SI}}\Vert p'_t - \hat{p}'_t\Vert,
\end{equation}
where $\hat{p}$ denotes the ground-truth label we assign, and $\lambda$ is set to 1 in our experiments. In this manner, the score personalized for this concept for each sample from $D_W$ can be predicted from the aesthetic scorer.

% the large-scale text-to-image already presents a good image encoder, so we can use this encoder to extract image features, this is how chad scorer is designed.

\subsubsection{Concept Matching Scorer}\label{method:concept_matching_scorer}

Since concept-matching in image retrieval are typically conducted on feature maps, we directly use the image encoder within the text-to-image model as the feature extractors and give out the matching score accordingly to the corresponding representation space. Let $R_T=\{r_1,r_2,\dots,r_{|\mathbf{X}_T|}\}$ be the feature map set extracted from $\mathbf{X}_T$, a concept-matching scorer $S_{con}$ can be formulated as:
\begin{equation}
    S_{con}(x)=\frac{1}{|\mathbf{X}_T|}\sum_{k=1}^{|\mathbf{X}_T|}\phi\left(r_x, r_k\right),
\end{equation}
where $r_x$ denotes the representation given by image-encoder on the given samples $x$, when function $\phi(r_x,r_k)$ is used to measure the similarity between sample $x$ and feature map $r_k$.

People has proposed several variants for $\phi(\cdot,\cdot)$ in this similarity evaluation, including VLAD~\cite{jegou2010aggregating}, Set distance~\cite{iscen2018mining} and Classification~\cite{boudiaf2020unifying}, which we modified to fit into our concept matching scorer:
\begin{itemize}
    \item By setting $\phi\left(r_x, r_k\right)=\psi(r_x, r_k)\exp\left(-\Vert r_x-r_k\Vert\right)$, where $\psi(r_x, r_k)=1$ if $r_k$ is the closet representation for $r_k$ and is set to 0 otherwise. VLAD regards the extracted representations for $\mathbf{X}_T$ as a codebook and maps each image to its nearest code.
    \item Set difference mines correlated samples by comparing their set distance, where $S_{con}(x)=\exp\left(-\min_{\mathbf{X}_T\in R_T}\Vert d_x - \mathbf{X}_T\Vert\right)$.
    \item Classification locates relevant samples by attaching and training another fully-connected network to the image coder and performs binary classification. By regarding $\mathbf{X}_T$ as positive samples and $D_{TG}\cup D_{SI}$ (proposed in~\ref{method:aesthetic_scorer}) as negative sample set, this can also be achieved with probabilistic outputs.
\end{itemize}
Note that samples within $\mathbf{X}_T$ are guaranteed to be clean and clear samples, this score is sufficient to quantify whether the object~(if exists) in the given image distinguish itself from other photographic components and match the given concept.

\subsubsection{Dual Scorer}\label{method:dual_scorer}

After calculating the aesthetic score and concept-matching score for each image, we combine these terms to form the final information score $S_{dual}(x)=F\left(S_{aes}(x), S_{con}(x)\right)$, where $F$ denotes a combination scheme and can be adjusted to serve different purposes~(with details explained in the following section). Meanwhile, note that the quality of embeddings can also be judged by their generated images, we also evaluate an embedding $e$ with this scoring system:
\begin{equation}
    S_{dual}(e)=\frac{1}{D_e}\sum_{x_e\in D_e}S_{dual}(x_e),
    \label{eq:embedding}
\end{equation}
where $D_e$ is the set of images generated by the text-to-image model according to embedding $e$.
At this stage, since the scoring system can both evaluate the quality of individual images and embeddings, we name this a "dual scorer".
% whether dual space theories can be added?

\subsection{Dual Selective Active Training}\label{method:dual_selective_active_training}

With the scoring system completed above, we are able to conduct our dual selective active training paradigm.
A naive way to incorporate the scoring system into the active learning paradigm is to use a fixed training schedule and move the top-ranked samples from $D_W$ to $\mathbf{X}_T$ for the next training cycle. Nevertheless, this strategy also results in unnecessary details or incorrect elements introduced into embeddings, as shown in Figure~\ref{fig:intro_example_comparison_2}. Though the scoring system does select samples with good quality, it fails to find samples that can further enhance the embedding. 
% 是否要配图强调如果不用动态的paradigm，而是单纯地根据得分选样本且schedule固定会怎么样

Since embedding evaluation and data acquisition serves different objectives, we apply different schemes when scoring embedding/samples. In particular, a good embedding should procedure images with both high aesthetics and object clarity, when good images for the next cycle should make up for the final embedding at the current cycle. 
To better select samples that further enhance the quality of embeddings, we propose a dual selective active training paradigm that couples embedding evaluation/selection and data acquisition as follows.

\subsubsection{Embedding Evaluation and Selection}\label{method:embedding_selection}
We measure the quality of an embedding through the aesthetic scores and concept-matching scores on its generated data batch, in which these two factors are equally important.
Given a embedding set $E=\{e_1,e_2,\dots,e_v\}$, we generate a evaluation set $D_{e_i}$ for each embedding $e_i$. Then, we use the dual scoring system to calculate the quality score for each generated data point:
\begin{equation}
    S_{dual}(x_e)=10\sin\left(\frac{\pi}{20}S_{aes}\left(e\right)\right)\sin\left(\frac{\pi}{20}S_{con}\left(e\right)\right). \label{eq:embedding_generated_image}
\end{equation}
% provide illustrations for using this function
This function changes rapidly when individual scores become close to 5.0, when 5.0 is exactly the average score that scorers tend to offer to most images, consistent with our need to quickly distinguish good examples from average ones. When one score draws near 10.0, the dual scorer become less sensitive to this score and will focus more on another factor. Last and perhaps more important, this score attains higher value when the two scores becomes close, which explicitly emphasize that embeddings that balancing the two factors are of better quality.
With the embedding score deduced then calculated according to Eq.~\ref{eq:embedding}, we manage to select the best version of embedding $e^*=\argmax_{e\in E}S_{dual}(e)$ among the embedding set $E$.

\subsubsection{Embedding Training Schedule}\label{method:schedule}

As the number of training samples increases, the quality of selected samples at later cycles might be lower, and a fixed schedule may introduce some unnecessary details within these images~(such as watermarks, borders, disturbing objects, etc.). But these subsequent samples with relatively lower quality do contain some good photographic that can help the embedding evolve. Actually, the potential problems can be alleviated by carefully-designed schedules.

We first train the embedding for $I$ epochs, and save an embedding version $e_i$ per $I_{step}$ epochs, together with its corresponding generated images, constituting a sub-cycle. When this sub-cycle is completed, we filter out the embedding with the highest quality based on the score in Sec.~\ref{method:embedding_selection}. If the selected embedding has the most training epochs across all versions, we keep the learning rate and conduct the next sub-cycle, otherwise we will reduce the learning rate. 
Note that if the embedding quality of this cycle is not as good as that of the previous cycle (because of the quality degradation caused by introducing some unnecessary details), the initial learning rate will be reduced, which help avoid introducing disturbing elements led by some samples with insufficient quality.
The sub-cycles will be continuously conducted until the minimum learning rate is reached or the embedding quality no longer increases.
The cycle in in Figure \ref{fig:intro_example_comparison_2}(b) offers an intuitive illustration for how \NAME{} make the schedule.

\subsubsection{Data Acquisition}\label{method:data_selection}

After getting the final embedding $e$ by carefully scheduling embedding training and selecting the best version among them, we select the most suitable samples for the next-cycle training.
Notice that whether newly selected images enhance the embedding depends on both the quality and the embedding, we ought to adjust our preferences according to the embedding. In more detail, when the embedding has high aesthetics but does not guarantee object clarity, samples with high concept-matching scores better enhance the embedding; when the embedding fails to exhibit some photographic attributes consistent with human, samples with high aesthetics are preferred. To implement this preference, our acquisition score for data in web-crawled set is:
\begin{equation}
    \begin{aligned}
        S_{dual}(x) &= (1-\sin(\frac{\pi}{20}S_{aes}(e)))S_{aes}(x) \\
        &+ (1-\sin(\frac{\pi}{20}S_{con}(e)))S_{con}(x).
    \end{aligned}
\end{equation}

After selecting top-K data accordingly to this score based on embedding quality, we assign a lowered aesthetic score to them:
\begin{equation}
    \hat{p}_x = 10.0 - \frac{N_{current}}{N_{total}}(10.0 - p_x),
\end{equation}
where $p_x$ denotes the score given by a generic aesthetic scorer, $N_{total}$ represents the number of total active learning cycles, when $N_{current}$ indicates the current cycle. Note that the newly-selected images typically have lower quality than those from earlier cycles, we assign progressively lowered score to them as learning cycle proceeds.

Finishing the active selection step for both embedding and next-cycle images, we repeat the loop above to fine-tune the scorers and the embedding on the updated training set $\mathbf{X}_T$.

\fi
